Multi-Task Imitation Learning for Linear Dynamical Systems

We study representation learning for efficient imitation learning over linear systems. In particular, we consider a setting where learning is split into two phases: (a) a pre-training step where a shared $k$-dimensional representation is learned from $H$ source policies, and (b) a target policy fine-tuning step where the learned representation is used to parameterize the policy class. We find that the imitation gap over trajectories generated by the learned target policy is bounded by $\tilde{O}\left( \frac{k n_x}{HN_{\mathrm{shared}}} + \frac{k n_u}{N_{\mathrm{target}}}\right)$, where $n_x > k$ is the state dimension, $n_u$ is the input dimension, $N_{\mathrm{shared}}$ denotes the total amount of data collected for each policy during representation learning, and $N_{\mathrm{target}}$ is the amount of target task data. This result formalizes the intuition that aggregating data across related tasks to learn a representation can significantly improve the sample efficiency of learning a target task. The trends suggested by this bound are corroborated in simulation.

==> appx_data_guarantee_v2.tex <==
 \section{WIP: Source guarantee v2} 
    



    
% \begin{proposition}
%     \label{lem: source controller concentration v2}
%     Under the setting of Theorem~\ref{thm:main}, with probability at least $1-\frac{\delta}{5}$,
%     \begin{align*}
%         \sum_{h=1}^H \norm{\Xdata^{(h)} \paren{\hat F^{(h)} \hat \Phi - F^{(h)}_\star \Phi_\star}^\top}_F^2 \lesssim \bar \sigma_z^2 \paren{k n_u H + kn_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}}  + \log\paren{\frac{1}{\delta}}}.
%     \end{align*}    
% \end{proposition}
% \begin{proof}

% \end{proof}

==> backup_sc.tex <==
\section{Sample Complexity of Multi-Task Imitation Learning}
\label{s: sample complexity}
%\Bruce{Subgaussian input and covariance domination are implicit from our assumptions on the noise. Covariance domination should be replaced just by using the ratio of maximum eignevalue to minimum eigenvalue.}
\sloppy



\st{move the proof summary to later (possibly appendix). show assumptions and results first.}
Toward establishing favorable guarantees on transfer imitation learning, we summarize the proof by the following main components:
\begin{enumerate}[noitemsep, nolistsep, leftmargin=*]
    \item In order to address the autocorrelated nature of the states along a given trajectory, we demonstrate that the empirical state covariance for each task along a given trajectory still concentrates to the true covariance. This gives us an additional statistical \textit{gain}
    %%SL.11.24: I don't get what the word "gain" means in this context
    through the trajectory length $T$.
    \item We then show that empirical minimizing representation and weights $\hat \Phi, \hat F^{(1)}, \dots, \hat F^{(H)}$ for problem \eqref{eq: pretraiing} concentrate to the true source controllers.
    \item We then show that the ERM target task weights $\hat F^{(H+1)}$ from solving problem \eqref{eq: target training} in conjunction with the representation $\hat \Phi$ derived from source tasks \eqref{eq: pretraiing} concentrate to the expert target controller.
    
    % \item We extract high probability bounds on both the target task controller error, and the excess risk on target task data generated by the expert trajectory. 
    \item The prior steps provide favorable guarantees on the imitation error between the true and learned target task controller $K^{(H+1)} - \hat K = F_\star^{(H+1)} \Phi_\star - \hat F^{(H+1)} \hat \Phi$. However, the imitation error is measured along expert target task trajectories, whereas we are interested in the closed-loop behavior of the learned controller $\hat K$. To that end, we demonstrate the tracking error between the closed-loop expert and learned states $\norm{x_\star[t] - \hat x[t]}$ scales directly with the imitation error $\norm{K^{(H+1)}x_\star[t] - \hat Kx_\star[t]}$.
    
    % \item We synthesize the controller error bound and the excess risk bound to bound the imitation loss on new rollouts. 
\end{enumerate}

\noindent Before proceeding, we note that in order to derive any useful information from source tasks for a downstream task, the source tasks must satisfy some notion of \textit{task diversity} that sufficiently covers the downstream task. Toward quantifying task diversity, we introduce the following notions of source tasks covering the target task.
% \st{This is not a new definition right? should reference du's paper.}
\begin{definition}[target task covariance coverage \citep{du2020few}]
\label{def: target task covariance coverage}
Let us define $c > 0$ to be the largest value where 
\begin{align}
    \label{eq: target task covariance coverage}
    \Sigma_x^{(h)} \succeq c \Sigma_x^{(H+1)} \quad \forall h \in [H].
\end{align}
Note that $c \geq \min_h \frac{\lambda_{\min}(\Sigma_x^{(h)})}{\lambda_{\max}(\Sigma_x^{(H+1)})} > 0$, by our assumption that $\Sigma_w^{(h)} \succ 0$ for all $h \in [H]$.   
\end{definition}
\Cref{def: target task covariance coverage} captures the degree to which the closed-loop distribution of states for each source task aligns with that of the target task, i.e.\ how much excitation states generated by each source task provides relative to the target task. We then introduce the following notion of task similarity between the source and target task weights, which generalizes the well-conditioning assumptions in \cite{du2020few} and \cite{tripuraneni2021provable}.
% \st{State that this is a generalization of du's assumption up front.}
\begin{assumption}[diverse source controllers] 
    \label{as: diverse source controllers}
We assume the target task weights $F_\star^{(H+1)}$ and the stacked source task weights $\Fdata_\star := \bmat{\paren{F_\star^{(1)}}^\top & \cdots & \paren{F_\star^{(H)}}^\top } \in \R^{k \times n_uH}$ satisfy
\begin{align}\label{eq: diverse source controllers}
    % \frac{\norm{F^{(H+1)}}_2^2}{\sigma_k^2\paren{\Fdata}} \leq \calO\paren{\frac{1}{H}}.
    \norm{\paren{\Fdata_\star^\dagger}^\top F^{(H+1)}}_2^2 \leq \calO\paren{\frac{1}{H}}.
\end{align}
\end{assumption}
% \Thomas{insert somewhat precise explanation of what this means}.
\Cref{as: diverse source controllers} essentially states that the alignment and loadings of the singular spaces between the stacked source task weights and target task weights closely match, along the low-dimensional representation axis. For example, if $F_\star^{(h)} = F_\star^{(H+1)}$ for each $h \in [H]$, the RHS of~\eqref{eq: diverse source controllers} is precisely $1/H$.
We note that this assumption subsumes and is somewhat more geometrically informative than a direct bound on the ratio of singular values, e.g.\ $\sigma_{\max}^2(F_\star^{(H+1)})/\sigma_k^2(\Fdata_\star) \leq \calO(1/H)$, which would follow by naively extending the well-conditioning assumptions of the weights in \cite{du2020few} and \cite{tripuraneni2021provable}. Notably, such a condition might not be satisfied even if $F_\star^{(h)} = F_\star^{(H+1)}$, $\forall h \in [H]$. \Thomas{lmk if more explanation needed (currently commented out)}
% Given $\norm{F^{(H+1)}_\star}^2_F = C$ this would implicitly require $\norm{F^{(h)}_\star}^2_F = \Omega(C)$ for all $h \in [H]$ and $\sigma_{\max}^2(F_\star^{(H+1)}) \leq \calO\paren{\frac{C}{k}}$, $\sigma_k^2(\Fdata_\star) = \Omega\paren{\frac{CH}{k}}$, which essentially says the singular values of controller weights have to be distributed approximately evenly. 
\st{Can we give an explicit example in a footnote?}
\Thomas{if target F has nullspace...}
We are now ready to present our main theoretical results.
% \begin{assumption}[normalization]
% \label{as: normalized weights}
%     We assume that the controller specific maps satisfy the following requirement on their Frobenius norm:
%     \[
%         \norm{F_\star^{(h)}}_F = \Theta(m) \qquad \forall 1\leq h \leq H+1.
%     \]
% \end{assumption}
% \begin{assumption}
%     The matrix 
% \[F_\star = \bmat{\paren{F^{(1)}_\star}^\top & \paren{F^{(2)}_\star}^\top & \dots & \paren{F^{(H)}_\star}^\top} \in \R^{k \times mH}\]
% satisfies 
%     \begin{align*}
%         \sigma_k^2\paren{\bmat{F^{(1)}_\star & F^{(2)}_\star &\dots F^{(H)}_\star}} \geq \Omega\paren{\frac{mH}{k}}.
%     \end{align*}
% \end{assumption}
% \begin{assumption}[distribution of target controller] 
%     \label{as: distribution of target controller}
%     % Let each row of $F^{(H+1)}_\star$ be sampled independently from some distribution $\nu$, which satisfies the property
%     % \[
%     %     \norm{\Ex_{f \sim \nu}\brac{ff^\top}}_F \leq O\paren{\frac{1}{k}}.
%     % \]
%     % The joint distribution will be denoted $\nu_F$. 
%     The spectral norm of the target controller weights $F^{(H+1)}_\star$ satisfies
%     \begin{align*}
%         \norm{F_\star^{(H+1)}}_2 \leq \calO\paren{\frac{m}{k}}.
%     \end{align*}
% \end{assumption}



\subsection{Concentration of Empirical Covariance Matrices}

If we were to rely on standard statistical learning tools based on independence, we would only see statistical gains from the number of trajectories $N_1 H$ and $N_2$. Therefore, the first step in establishing our desired bounds is to show that, analogous to the i.i.d.\ setting, the empirical covariance matrix $\frac{1}{T}\sum_{t=0}^{T-1} x^{(h)}[t]x^{(h)}[t]^\top$ concentrates towards the true covariance matrix $\Sigma_x^{(h)}$ for any given task $h \in [H+1]$, thereby allowing us to extract statistical gains from the trajectory length $T$ downstream. To that end, we adapt tools from \cite{jedra2020finite} for linear system identification, which leads to the following covariance concentration results.
\begin{restatable}{lemma}{SourceCovarianceConcentration}
    \label{lem: source covariance concentration}
    Suppose $N_1 T \geq C \max_h \calJ\paren{A + B K^{(h)}}^2 \kappa\paren{\Sigma_x^{(h)}} (n_x + \log(H/\delta))$ for $\delta \in (0,1)$, where $C$ is a universal numerical constant. Then with probability at least $1-\frac{\delta}{10}$ over the states $\Xdata^{(1)}, \dots, \Xdata^{(H)}$ in the source tasks, we have
    \[
        0.9 \Sigma_x^{(h)} \preceq \frac{1}{N_1 T} \paren{\Xdata^{(h)}}^\top \Xdata^{(h)} \preceq 1.1 \Sigma_x^{(h)}, \qquad \forall h \in [H].
    \]
\end{restatable}
\begin{restatable}{lemma}{TargetCovarianceConcentration}
    \label{lem: target covariance concentration}
    Suppose $N_2 T \geq  C\calJ\paren{A + B K^{(H+1)}}^2 \kappa\paren{\Sigma_x^{(H+1)}}(k + \log(1/\delta))$ for $\delta \in (0,1)$, where $C$ is a universal numerical constant. Then for any given matrix $\Phi \in \R^{n_x \times 2k}$ independent of $\Xdata^{(H+1)}$, with probability at least $1-\frac{\delta}{10}$ over $\Xdata^{(H+1)}$ we have
    \[
        0.9 \Phi^\top \Sigma_x^{(H+1)} \Phi \preceq \frac{1}{N_2 T} \Phi^\top \paren{\Xdata^{(H+1)}}^\top \Xdata^{(H+1)} \Phi \preceq 1.1 \Phi^\top \Sigma_x^{(H+1)} \Phi. 
    \]
\end{restatable}
Proofs and additional details for the above lemmas can be found in \Cref{appendix: covariance concentration}. We observe that the sample complexity of the source tasks covariance concentration scales with the state dimension $n_x$, while that of the target task only scales with the representation dimension $k$. However, both sample complexities are hit by a factor scaling with closed-loop stability $\calJ\paren{A + B K}$, which quantifies a burn-in time requirement for learning over dependent covariates.
% \citep{yu1994rates, kuznetsov2017generalization}. \Thomas{cite more?}
% \st{This is more a burn-in time, since the ratios
% $0.9$ and $1.1$ are ultimately independent of the mixing time.}


\subsection{Target Task Excess Risk Guarantees}

The goal of this section is to show that learning controllers in this de-coupled manner through fitting a representation and target task weights leads to favorable generalization bounds on the excess risk of the learned controller inputs on the expert target task state distribution, analogous to the bounds on multi-task linear regression in \cite{du2020few, tripuraneni2021provable}. However, a key complicating factor in our setting is the fact that the input noise $z^{(h)}[t]$ enters the process, and thus the data $x^{(h)}[t]$ is causally dependent on the ``label noise''. In order to overcome this issue and preserve our statistical gains along time $T$, we leverage the theory of self-normalized martingales, in particular generalizing tools from \cite{abbasi2011online} to the matrix-valued setting. The full argument is detailed in \Cref{appendix: data guarantees}. This culminates in the following target task excess risk bound.
\begin{restatable}[target task excess risk bound]{theorem}{TargetTaskRiskBound}
\label{thm: target task excess risk bound}
    % For $\delta \in (0,1)$, suppose that the source data satisfies
    % $N_1 T \gg \max_h \calJ\paren{A + B K^{(h)}}^2 \kappa\paren{\Sigma_x^{(h)}} (n_x + \log(H/\delta))$ and the target data satisfies $N_2 T \gg   \calJ\paren{A + B K^{(H+1)}}^2 \kappa\paren{\Sigma_x^{(H+1)}}(k + \log(1/\delta))$. Then with probability at least $1-\delta$,
    Given $\delta \in (0,1)$, suppose that the sample requirements in \Cref{lem: source covariance concentration} and \Cref{lem: target covariance concentration} are satisfied. Define $\calP_{0:T-1}^{(H+1)}$ as the probability distribution over target task trajectories $(x^{(H+1)}[0], \cdots, x^{(H+1)}[T-1])$. Then with probability at least $1-\delta$, the excess risk of the learned representation $\hat{\Phi}$ and target task weights $\hat F^{(H+1)}$ is bounded by
    %Under the setting of Theorem~\ref{thm: final imitation gap bound}, the excess risk follows the following bound:
    \begin{align*}
        %  \Ex_{F^{(H+1)}_\star \sim \nu_F}\brac{\ER(\hat \Phi, \hat F^{(H+1)})} \lesssim \bar \sigma_z^2 \paren{\frac{k n \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{km +\log(\frac{1}{\delta})}{N_2 T}}. 
         \ER(\hat \Phi, \hat F^{(H+1)}) &:= \frac{1}{2 T} \Ex_{\calP_{0:T-1}^{(H+1)}} \brac{\sum_{t=0}^{T-1} \norm{(F_\star^{(H+1)} \Phi_\star - \hat F^{(H+1)} \hat \Phi) x^{(H+1)}[t]}_2^2} \\
         &\lesssim  \sigma_z^2 \paren{\frac{k n_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{kn_u +\log(\frac{1}{\delta})}{N_2 T}}. 
    \end{align*}
\end{restatable}
% \st{It would be good to clarify that the expectation in $\ER$ is
% over fresh realizations of $x^{(H+1)}[t]$ only, treating
% $\hat{F}^{(H+1)}, \hat{\Phi}$ as fixed.}

\subsection{Tracking Error Guarantees: Tackling Distribution Shift} 

As we are studying the pure offline imitation learning (``behavioral cloning'') setting, we do not assume that these controllers are optimizing any particular objective, and never consider a control objective function in our analysis.
% we do not make assumptions about the optimality of these controllers for any particular objective
 We also do not assume knowledge of any part of the dynamics beyond the provided (state, action)-pair trajectory data. Therefore, to understand the performance of the learned target controller in closed-loop, we are interested in bounding in high probability the deviation of states generated by the learned and expert target controller run in closed-loop. In other words, we bound the \textit{tracking error}. This requires us to address the challenging \textit{distribution shift} problem. \Thomas{can go to problem statement}


Transferring a bound on the excess risk of the target task $\ER(\hat \Phi, \hat F^{(H+1)})$ into a bound on the tracking error is non-trivial, due to the fundamental distribution shift between the expert trajectories seen during training and the trajectories generated by running the learned controller in closed-loop. 
% \st{I would condense the next two paragraphs into a sentence, 
% something like, ``we leverage the recent framework of Pfrommer et al.\ to bound the tracking error, making the necessary modifications
% to handle stochasticity. The details can be found in Appendix XYZ.''}
We leverage the recent framework of \cite{pfrommer2022tasil} to bound the tracking error, making the necessary modifications to handle stochasticity. A more detailed exposition can be found in \Cref{appendix: bounding imitation gap}.

Let us define the following notation denoting the state of the expert versus learned target task closed-loop systems: given a learned controller $\hat K = \hat F^{(H+1)} \hat \Phi$ from solving \eqref{eq: pretraiing} and \eqref{eq: target training}, for a given realization of randomness $x[0] \sim \calN(0, \Sigma_x^{(H+1)})$, $z[t] \sim \calN(0, \sigma_z^2 I)$, $w[t] \sim N(0, \Sigma_w^{(H+1)}), t = 0, \dots, T$, we write
\begin{align*}
    x_\star[t+1] &= (A + BK^{(H+1)}) x_\star[t] + Bz[t] + w[t], \quad x_\star[0] = x[0] \\
    \hat x[t+1] &= (A + B\hat K)\hat x[t] + Bz[t] + w[t],  \quad \hat x[0] = x[0].
\end{align*}
The following result provides a high probability bound on the closed-loop tracking error $\norm{x_\star[t] - \hat x[t]}$ for an i.i.d.\ sampled set of process randomness that scales with the excess risk of the learned controller, which formalizes the notion that low training error implies low test error, in spite of distribution shift. Let $\calP^\star_{1:T}$ and $\hat\calP_{1:T}$ denote the distributions of trajectories $\curly{x_\star[t]}_{t=1}^{T}$ and $\curly{\hat x[t]}_{t=1}^{T}$.
% \begin{restatable}[Target Imitation Error Bound]{theorem}{TargetImitationErrorBound} \label{thm: final imitation gap bound short}
% Let us choose constants 
% \begin{align*}
% \nu \in \paren{\rho(A + BK^{(H+1)}), 1}, \quad \tau := \sup_{k \in \N} \frac{\norm{\paren{A + BK^{(H+1)}}^k}_2}{\nu^k},
% \end{align*}
% which are guaranteed to exist by Gelfand's formula \citep[Corollary 5.6.13]{horn2012matrix}. Given the generalization bound on the excess risk of the learned representation and target task weights $(\hat\Phi, \hat F^{(H+1)})$ from \Cref{thm: target task excess risk bound} for a fixed failure probability $\delta \in (0,1)$, we propose the following bound on the tracking error. Assume we have sufficiently many samples $H, T, N_1, N_2$ such that
% \begin{equation*}
%     \bar \sigma_z^2 \paren{\frac{k n_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{kn_u +\log(\frac{1}{\delta})}{N_2 T}} \lesssim \frac{(1 - \nu)^2\lambda_{\min}\paren{\Sigma_x^{(H+1)}}}{\tau^2 \norm{B}^2_2}.
% \end{equation*}
% Then with probability greater than $1- \delta - \delta'$, for a new target task trajectory sampled with i.i.d.\ process randomness $x[0] \sim \Sigma_x^{(H+1)}$, $w[t] \sim \Sigma_w^{(H+1)}$, $t = 0, \dots, T-1$, the tracking error satisfies
% \begin{align}
%     \max_{1 \leq t \leq T} \norm{\hat x[t] - x_\star[t]}^2 &\lesssim \frac{\tau^2  \norm{B}^2_2}{(1-\nu)^2} \log\paren{\frac{T}{\delta'}} \mathrm{ER}(\hat{\Phi}, \hat W^{H+1}) \\
%     &\lesssim \frac{\bar \sigma_z^2 \tau^2  \norm{B}^2_2}{(1-\nu)^2} \log\paren{\frac{T}{\delta'}}  \paren{\frac{k n_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{kn_u +\log(\frac{1}{\delta})}{N_2 T}}.
% \end{align}
% % where the expert and learned trajectory states $\hat x[t]$ and $x_\star[t]$ are as defined in \Cref{prop: linear TaSIL guarantee}.

% \end{restatable}
\begin{restatable}[Target Imitation Error Bound]{theorem}{TargetImitationErrorBound} \label{thm: final imitation gap bound short}
Given the generalization bound on the excess risk of the learned representation and target task weights $(\hat\Phi, \hat F^{(H+1)})$ from \Cref{thm: target task excess risk bound} for a fixed failure probability $\delta \in (0,1)$, we propose the following bound on the tracking error. Define $A_{\mathsf{cl}} := A+BK^{(H+1)}$. Assume we have sufficiently many samples $H, T, N_1, N_2$ such that
\begin{equation*}
     \sigma_z^2 \paren{\frac{k n_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{kn_u +\log(\frac{1}{\delta})}{N_2 T}} \lesssim \frac{\lambda_{\min}\paren{\Sigma_x^{(H+1)}}}{\calJ\paren{A_{\mathsf{cl}}}^2\norm{B}^2_2}.
\end{equation*}
Then with probability greater than $1- \delta - \delta'$, for a new target task trajectory sampled with i.i.d.\ process randomness $x[0] \sim \Sigma_x^{(H+1)}$, $w[t] \sim \Sigma_w^{(H+1)}$, $t = 0, \dots, T-1$, the tracking error satisfies
\begin{align}
    \begin{split}\label{eq: Thm 3.2 high prob bound}
    \max_{1 \leq t \leq T} \norm{\hat x[t] - x_\star[t]}^2 &\lesssim \calJ\paren{A_{\mathsf{cl}}}^2\norm{B}^2_2 \log\paren{\frac{T}{\delta'}} \mathrm{ER}(\hat{\Phi}, \hat F^{(H+1)}) \\
    &\lesssim \sigma_z^2 \calJ\paren{A_{\mathsf{cl}}}^2\norm{B}^2_2 \log\paren{\frac{T}{\delta'}}  \paren{\frac{k n_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{kn_u +\log(\frac{1}{\delta})}{N_2 T}}.
    \end{split}
\end{align}
% where the expert and learned trajectory states $\hat x[t]$ and $x_\star[t]$ are as defined in \Cref{prop: linear TaSIL guarantee}.
Furthermore, for any cost function $h(\cdot)$ that is $L$-Lipschitz with respect to the trajectory-wise metric $d\paren{\vec x_{1:T}, \vec y_{1:T}} = \max_{1 \leq t \leq T} \norm{x[t] - y[t]}$, with probability greater than $1-\delta$ we have the following bound on the expected cost gap
\begin{align}\label{eq: Thm 3.2 expectation bound}
    \abs{\Ex_{\hat\calP_{1:T}}\brac{h(\hat{\vec x}_{1:T})} - \Ex_{\calP^\star_{1:T}}\brac{h(\vec x^\star_{1:T})}} &\lesssim L\calJ(A_{\mathsf{cl}})\norm{B} \sqrt{\log(T)} \sqrt{\mathrm{ER}(\hat{\Phi}, \hat F^{(H+1)})}.
\end{align}
% \Thomas{Furthermore, for any cost $h(\cdot)$ that is $L$-lipschitz wrt to metric, we have bound}

\end{restatable}

\begin{remark}
    The dependence of the tracking error bound in \eqref{eq: Thm 3.2 high prob bound} on the stability of the target-task closed-loop system through $\calJ(A_{\mathsf{cl}})$ is tight. Intuitively, less stable systems exacerbate the input errors from the learned controller. The formal construction of a lower bound is relegated to \Cref{appendix: bounding imitation gap}.
\end{remark}

\begin{remark}
    Some examples of Lipschitz $h(\cdot)$ include LQR state costs $h(\vec x_{1:T}) = \max_t \norm{Q^{1/2} x[t]}$ and regularized tracking costs $h(\vec x_{1:T}) = \max_t \norm{x[t] - x_{\mathrm{goal}}[t]} + \lambda \norm{Rx[t]}$. Since $\frac{1}{T}\sum_{t=1}^{T} \norm{x[t] - y[t]} \leq \max_{1 \leq t \leq T} \norm{x[t] - y[t]}$, \eqref{eq: Thm 3.2 expectation bound} holds with no modification for time-averaged costs $h(\cdot)$.
\end{remark}

% \st{What do you think about the following modification?
% Consider the metric $\rho(x, y) = \max_{1\leq t \leq T} \| x[t] - y[t] \|$, and let $W_\rho(\mathsf{P}^\star_{1:T}, \hat{\mathsf{P}}_{1:T})$
% denote the Wasserstein distance between the joint distribution of the
% expert and theh learned policy w.r.t. the $\rho$ metric.
% The result above (if you change it from wp at least $1-\delta'$
% to expected value), actually gives a bound on
% the $W_\rho$ distance (use Jensen's).
% Hence, by Kantorovich-Rubinstein Duality,
% for any function $f$ which is $1$-Lipschitz wrt $\rho$,
% \begin{align*}
%     |\Ex_{\mathsf{P}^\star_{1:T}} f - \Ex_{\hat{\mathsf{P}}_{1:T}} f|
% \end{align*}
% is upper bounded by your bound.
% Thus for any reasonable observable function (e.g. something
% that measures performance of system),
% you can argue that the learned system is close to the expert system.
% For example, consider $f(x) = \max_{1 \leq t \leq T} \| x[t] - x_{\mathrm{goal}} \| + R\|B x[t]\|$,
% which is some weighted combination of goal tracking and
% control effort.}


Consider the following joint metric on trajectories and controllers $K$:
\begin{align*}
    d\paren{\paren{\vec x_{1:T}, K_1}, \paren{\vec y_{1:T}, K_2}} &:= \max\curly{\max_{1\leq t \leq T} \norm{x[t] - y[t]}, \norm{K_1 - K_2}}, 
\end{align*}
i.e.\ a signal $\ell_\infty$ norm along the states of the trajectories augmented with controllers. Let us also define the (root) LQR cost defined on $\paren{\vec x_{1:T}, K_1}$
\begin{align*}
    h\paren{\paren{\vec x_{1:T}, K_1}} &:= \max_{1 \leq t \leq T} \sqrt{x[t]^\top
    \paren{Q + K^\top R K}x[t]} \\
    &= \max_{1 \leq t \leq T} \norm{\bmat{Q^{1/2} \\ R^{1/2} K} x[t]}.
\end{align*}
Our goal is to show that $h(\cdot)$ is essentially $L$-Lipschitz with respect to $d$. First, consider the following elementary inequality:
\begin{align*}
    \norm{M_1 x_1} - \norm{M_2 x_2} &= \norm{M_1 x_1} - \norm{M_1 x_2} + \norm{M_1 x_2} - \norm{M_2 x_2} \\
    &\leq \norm{M_1 (x_1 - x_2)} + \norm{(M_1 - M_2)x_2} \\
    &\leq \norm{M_1} \norm{x_1 - x_2} + \norm{x_2} \norm{M_1 - M_2} \\
    &\leq \max\curly{\norm{M_1}, \norm{x_2}} \cdot \max\curly{\norm{x_1 - x_2}, \norm{M_1 - M_2}}.
\end{align*}
Applying this to $h\paren{\paren{\vec x_{1:T}, K_1}} - h\paren{\paren{\vec y_{1:T}, K_2}}$, we get
\begin{align*}
    &h\paren{\paren{\vec x_{1:T}, K_1}} - h\paren{\paren{\vec y_{1:T}, K_2}} \\
    =\;& \max_{1 \leq t \leq T} \norm{\bmat{Q^{1/2} \\ R^{1/2} K_1} x[t]} - \max_{1 \leq t \leq T} \norm{\bmat{Q^{1/2} \\ R^{1/2} K_2} y[t]} \\
    \leq\;& \max_{1 \leq t \leq T} \norm{\bmat{Q^{1/2} \\ R^{1/2} K_1} x[t]} - \norm{\bmat{Q^{1/2} \\ R^{1/2} K_2} y[t]} \\
    \leq\;& \max_{1 \leq t \leq T} \max\curly{\norm{\bmat{Q^{1/2} \\ R^{1/2} K_1}}, \norm{y[t]}} \max\curly{\norm{x[t] - y[t]}, \norm{\bmat{Q^{1/2} \\ R^{1/2} K_1} - \bmat{Q^{1/2} \\ R^{1/2} K_2}}} \\
    \leq\;& \sqrt{\lambda_{\max}(R)} \max\curly{\norm{\bmat{Q^{1/2} \\ R^{1/2} K_1}}, \max_t \norm{y[t]}} \cdot \max\curly{\max_t \norm{x[t] - y[t]}, \norm{K_1 - K_2}} \\
    =:\;&\sqrt{\lambda_{\max}(R)} \max\curly{\norm{\bmat{Q^{1/2} \\ R^{1/2} K_1}}, \max_t \norm{y[t]}} \cdot d\paren{\paren{\vec x_{1:T}, K_1}, \paren{\vec y_{1:T}, K_2}}.
\end{align*}
Therefore, it remains to bound the factor
\[
\max\curly{\norm{\bmat{Q^{1/2} \\ R^{1/2} K_1}}, \max_t \norm{y[t]}}.
\]
However, without further specification, $\norm{K_1}$ and $\norm{y[t]}$ are not bounded. Observe that when we evaluate the expected LQR costs over learned and expert trajectories, the respective controllers $\hat K$ and $K^{(H+1)}$ are fixed and thus are independent from $\hat\calP_{1:T}$ and $\calP^{\star}_{1:T}$. Therefore, it suffices to restrict the domain to the line
\[
\calK := \curly{K : K = \mu \hat K + (1-\mu) K^\star,\;0\leq \mu \leq 1}.
\]
As for $\max_t \norm{y[t]}$, let us prescribe an almost-sure uniform upper bound that defines the domain of trajectories $\vec y_{1:T}$
\[
\norm{y[t]} \leq M,\quad t = 0,\dots, T,
\]
which we will instantiate later. Under this specification of the domains of $K$ and $\vec y_{1:T}$, we can upper bound the Lipschitz constant of the root-LQR cost $h(\cdot)$ with respect to $d$:
\begin{align*}
    \norm{h}_{\mathrm{Lip}} &:= \sup_{\substack{\vec x_{1:T}, \norm{\vec y_{1:T}}_\infty \leq M \\
    K_1, K_2 \in \calK} } \frac{\abs{h\paren{\paren{\vec x_{1:T}, K_1}} - h\paren{\paren{\vec y_{1:T}, K_2}}}}{d\paren{\paren{\vec x_{1:T}, K_1}, \paren{\vec y_{1:T}, K_2}}} \\
    &\leq \sqrt{\lambda_{\max}(R)} \max\curly{\norm{\bmat{Q^{1/2} \\ R^{1/2} K_1}}, \max_t \norm{y[t]}} \\
    &\leq \sqrt{\lambda_{\max}(R)} \max\curly{\sqrt{\lambda_{\max}(Q)} + \sqrt{\lambda_{\max}(R)} \max_{K \in \calK} \norm{K} ,  \;M} \\
    &\leq \max\curly{ \sqrt{\lambda_{\max}(Q)\lambda_{\max}(R)} + \lambda_{\max}(R) \max\curly{\norm{\hat K}, \norm{K^{(H+1)}}},\;\; \sqrt{\lambda_{\max}(R)} M  }.
\end{align*}
It remains to instantiate $M$. Toward this end, let us instantiate the (marginal) distributions on which $(\vec x_{1:T}, K_1)$ and $(\vec y_{1:T}, K_2)$ are defined. Let $\vec x_{1:T} \equiv \hat {\vec x}_{1:T}$, $K_1 \equiv \hat K$, $\vec y_{1:T} \equiv \vec x^\star$, $K_2 \equiv K^{(H+1)}$, such that we may define the distributions $(\vec{\hat x}_{1:T}, \hat K) \sim \hat \calP_{1:T} \otimes \delta_{\hat K}$, $(\vec x^\star_{1:T}, K^{(H+1)}) \sim \calP^\star_{1:T} \otimes \delta_{K^{(H+1)}}$, where $\delta$ denotes the Dirac delta distribution. We note that since $\hat K$ and $K^{(H+1)}$ are assumed fixed while rolling out new trajectories, these distributions are well-defined. For simplicity, we will omit the Dirac delta going forward. Therefore, by our choice of definitions, to find $M$ is sneakily reduced to finding a (high-probability) upper bound on the \textit{expert} trajectories $\vec x^\star_{1:T}$. We can achieve this by once again re-hashing the Hanson-Wright inequality. For a desired success probability $1-\delta'$ that we would like the event
$\curly{\max_{1 \leq t \leq T} \norm{x_\star[t]} \leq M }$
to hold, we apply \Cref{prop: Hanson-Wright for Gaussians} with $R = \paren{\Sigma^{(H+1)}_x}^{1/2}$ and a union bound over $1 \leq t \leq T$ to get
\begin{align*}
    \prob\brac{\max_{1 \leq t\leq T}\norm{x_\star[t]}^2 \geq (1 + \varepsilon) \trace\paren{\Sigma_x^{(H+1)}}  } &\leq T \exp\paren{- \frac{1}{\sqrt{3}}\min\curly{\frac{9\varepsilon^2}{64}, \frac{3\varepsilon}{8} } \frac{\norm{R}_F^2}{\norm{R}^2}} \\
    &\leq \delta'.
\end{align*}
Inverting this bound finds that
\begin{align*}
    \varepsilon &:= 
    % \frac{8\sqrt{3}}{3} \frac{\kappa\paren{\Sigma^{(H+1)}_x}}{n_x}\log\paren{\frac{T}{\delta'}}
    % \geq 
    \frac{8\sqrt{3}}{3} \frac{\lambda_{\max}\paren{\Sigma^{(H+1)}_x}}{\trace\paren{\Sigma^{(H+1)}_x}}\log\paren{\frac{T}{\delta'}},
\end{align*}
is sufficient to satisfy the desired failure probability. Therefore, setting
\begin{equation}\label{eq: truncation bound}
M = \sqrt{1 + \frac{8\sqrt{3}}{3} \frac{\lambda_{\max}\paren{\Sigma^{(H+1)}_x}}{\trace\paren{\Sigma^{(H+1)}_x}}\log\paren{\frac{T}{\delta'}}} \leq 3 \sqrt{\frac{\lambda_{\max}\paren{\Sigma^{(H+1)}_x}}{\trace\paren{\Sigma^{(H+1)}_x}}\log\paren{\frac{T}{\delta'}}}, \quad \text{for }\delta' < 1/3
\end{equation}
we have over trajectories $\vec x^\star_{1:T}$ the event
\[
\prob\brac{\max_{1 \leq t \leq T} \norm{x_\star[t]} \leq M} =: \prob\brac{\calA(M)} \geq 1- \delta'.
\]
In particular, defining the truncated process
\begin{align*}
    \bar{\vec x}^\star_{1:T} &:= \vec x^\star_{1:T} \ones_{\calA(M)},
\end{align*}
we can write the expected cost gap as
\begin{align*}
    &\abs{\Ex_{\hat\calP_{1:T}}\brac{h\paren{\paren{\vec \hat x_{1:T}, \hat K}}} - \Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\vec x^\star_{1:T}, K^{(H+1)}}}} } \\
    \leq\;&\abs{\Ex_{\hat\calP_{1:T}}\brac{h\paren{\paren{\vec \hat x_{1:T}, \hat K}}} - \Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\vec x^\star_{1:T}, K^{(H+1)}}} \ones_{\calA(M)} }  } + \abs{\Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\vec x^{\star}_{1:T}, K^{(H+1)}}} \ones_{\calA(M)^c}  }} \\
    \leq\;&\abs{\Ex_{\hat\calP_{1:T}}\brac{h\paren{\paren{\vec \hat x_{1:T}, \hat K}}} - \Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\bar{\vec x}^\star_{1:T}, K^{(H+1)}}} }  } + \sqrt{\Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\vec x^{\star}_{1:T}, K^{(H+1)}}}^2 }} \cdot \sqrt{\delta'},
\end{align*}
where the last line comes from applying Cauchy-Schwarz. Since the first term is now conditioning on the bounded expert trajectory event, we can compute the Lipschitz constant for a given bound $M$ (that we will determine in hindsight). It remains to bound the second term. We observe that this reduces to computing the closed-loop LQR cost of the expert system and an application of the maximal inequality (cf.\ \Cref{prop: max-to-avg excess risk}):
\begin{align}
    \Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\vec x^{\star}_{1:T}, K^{(H+1)}}}^2 } &= \Ex_{\calP^\star_{1:T}}\brac{\max_{1 \leq t \leq T} x^\star[t]^\top \paren{Q + {K^{(H+1)}}^\top R K^{(H+1)}} x^\star[t] } \nonumber \\
    &\leq 3\paren{1 + \log(T)}\Ex_{\calP^\star_{1:T}}\brac{\frac{1}{T}\sum_{t=1}^{T}x^\star[t]^\top \paren{Q + {K^{(H+1)}}^\top R K^{(H+1)}} x^\star[t] } \nonumber \\
    &= 3\paren{1 + \log(T)} \trace\paren{\paren{Q + {K^{(H+1)}}^\top R K^{(H+1)}} \Sigma_x^{(H+1)}}. \label{eq: expert LQR cost}
\end{align}
All that is left is to choose a $\delta'$ that balances between the first and second terms, where by \eqref{eq: truncation bound} the first term scales with $\log(1/\delta')$ and the second with $\sqrt{\delta'}$. Observe that $a\log(1/\delta') + b\sqrt{\delta'}+c$ for $a, b, c > 0$ attains its minimum at $\delta' = \frac{4a^2}{b^2}$. We instantiate the scaling of the terms $a,b$. We apply Kantorovich-Rubinstein duality to find
\begin{align*}
    &\abs{\Ex_{\hat\calP_{1:T}}\brac{h\paren{\paren{\vec \hat x_{1:T}, \hat K}}} - \Ex_{\calP^\star_{1:T}}\brac{h\paren{\paren{\bar{\vec x}^\star_{1:T}, K^{(H+1)}}} }  } \\
    \leq\;& \norm{h}_{\mathrm{Lip}} \Ex_{\Gamma(\hat\calP_{1:T}, \calP^\star_{1:T})}\brac{d\paren{(\vec {\hat x}_{1:T}, \hat K), (\vec x^\star_{1:T}, K^{(H+1)}) }} \\
    \leq\;& \norm{h}_{\mathrm{Lip}} \Ex_{\Gamma(\hat\calP_{1:T}, \calP^\star_{1:T})}\brac{\max\curly{\max_{1\leq t \leq T} \norm{\hat x[t] - x^\star[t]}, \norm{\hat K - K^{(H+1)}} }  } \\
    \leq\;& \norm{h}_{\mathrm{Lip}} \paren{\Ex_{\Gamma(\hat\calP_{1:T}, \calP^\star_{1:T})}\brac{\max_{1\leq t \leq T} \norm{\hat x[t] - x^\star[t]} } + \norm{\hat K - K^{(H+1)}}},
\end{align*}
where $\Gamma(\hat\calP_{1:T}, \calP^\star_{1:T})$ denotes the coupling described in \eqref{eq: identical coupling} where the learned and expert trajectories are evaluated on the same realizations of randomness. Since we are evaluating on the success event of learning the controller $\hat K$ for a given failure probability $\delta$, \Cref{thm: target task excess risk bound} gives us
\begin{align*}
    \ER(\hat \Phi, \hat F^{(H+1)}) &= \frac{1}{2} \trace\paren{(\hat K - K^{(H+1)})\Sigma_x^{(H+1)} (\hat K - K^{(H+1)})^{\top}}\\
     % &\lesssim  \sigma_z^2 \paren{\frac{k n_x \log\paren{N_1 T \frac{\bar \lambda}{\underline{\lambda}}} }{ cN_1 T H} + \frac{kn_u +\log(\frac{1}{\delta})}{N_2 T}} \\
     \implies \norm{\hat K - K^{(H+1)}} &\leq \lambda_{\min}\paren{\Sigma_x^{(H+1)}}^{-1/2} \sqrt{\ER(\hat \Phi, \hat F^{(H+1)})},
\end{align*}
while on the other hand \Cref{thm: in-expectation imitation gap full} yields
\begin{align*}
    \Ex_{\Gamma(\hat\calP_{1:T}, \calP^\star_{1:T})}\brac{\max_{1\leq t \leq T} \norm{\hat x[t] - x^\star[t]} } &\leq 2\sqrt{3} \calJ(A_{\mathsf{cl}})\norm{B} \sqrt{1+\log(T)} \sqrt{\mathrm{ER}(\hat{\Phi}, \hat F^{(H+1)})}. 
\end{align*}
Defining $C = \lambda_{\min}\paren{\Sigma_x^{(H+1)}}^{-1/2} + 2\sqrt{3} \calJ(A_{\mathsf{cl}})\norm{B} \sqrt{1+\log(T)}$ and recalling the bound on $\norm{h}_{\mathrm{Lip}}$ and $M$ \eqref{eq: truncation bound}, we may set
\[
a = 3 \sqrt{\lambda_{\max}(R)}\sqrt{\frac{\lambda_{\max}\paren{\Sigma^{(H+1)}_x}}{\trace\paren{\Sigma^{(H+1)}_x}}} C \sqrt{\mathrm{ER}(\hat{\Phi}, \hat F^{(H+1)})},
\]
and we set
\begin{align*}
    b := 3C \sqrt{\lambda_{\max}\paren{Q + {K^{(H+1)}}^\top R K^{(H+1)}}} \sqrt{\trace\paren{\Sigma^{(H+1)}_x}},
\end{align*}
which by definition upper bounds the (square-root of) expression in \eqref{eq: expert LQR cost}.
